Attentive Knowledge-aware Graph Convolutional Networks with Collaborative Guidance for Personalized Recommendation

To alleviate data sparsity and cold-start problems of traditional recommender systems (RSs), incorporating knowledge graphs (KGs) to supplement auxiliary information has attracted considerable attention recently. However, simply integrating KGs in current KG-based RS models is not necessarily a guarantee to improve the recommendation performance, which may even weaken the holistic model capability. This is because the construction of these KGs is independent of the collection of historical user-item interactions; hence, information in these KGs may not always be helpful for recommendation to all users. In this paper, we propose attentive Knowledge-aware Graph convolutional networks with Collaborative Guidance for personalized Recommendation (CG-KGR). CG-KGR is a novel knowledge-aware recommendation model that enables ample and coherent learning of KGs and user-item interactions, via our proposed Collaborative Guidance Mechanism. Specifically, CG-KGR first encapsulates historical interactions to interactive information summarization. Then CG-KGR utilizes it as guidance to extract information out of KGs, which eventually provides more precise personalized recommendation. We conduct extensive experiments on four real-world datasets over two recommendation tasks, i.e., Top-K recommendation and Click-Through rate (CTR) prediction. The experimental results show that the CG-KGR model significantly outperforms recent state-of-the-art models by 1.4-27.0% in terms of Recall metric on Top-K recommendation.

==> memo.tex <==
\section{memo}

{\color{blue}
9 pages + unlimited reference.


Re-run BookCrossing (mainly focused on the LR tuning)

1. Method Figure
2. difference vs. (KGCN KGAT CKAN) (highlight)

Trust-able: CF (user, item) +  [Fine-grained]-Attention method: external KG  <(u,v),h,r,t>

Motivation: robustness (noise)
Proposed method: xxx Fine-grained 

Full 4 dataset
Ablation study + analysis:
- -User+information
- -item+information
- -entity+information
- Only CF
- Leverage KGCN Attention: <u,r,t>
- (h, r, t)
- CKAN (attention method)
- [Fine-grained]-Attention method: external KG  <(u,v),h,r,t>

Supplementary:
Full 4 dataset: Top-k Recall@20
LastFM (corrupted triplets: 0.5 corrupt kg + 0.5 corrupt link)
show robustness: noise ratio (5\%, 10\%, 15\%, 20\%)



Most unique: <(u,v),h,r,t>

1. (user neighbor, item neighbor aggregation)
2. fine-grained attention, for each <user, item> rewight external knowledge



20210107:

1. CF + (corrupted triplets 10% 20% ... 80%) more robust

<h, r, t> -> <h', r, t> or <h, r, t'>
<i, e> -> <i, e'>
2. case study (visuliaze)
3. ablation study
f(<u, i>, h, r, t) KGCN -> f(u, r) KGAT -> f(u, r, i) + (i, r, e) CKAN -> f(i, r, e) + f(u, r, e)
Agg U
Agg I



Explicit Integration of external Knowledge for robust personalized recommendation 

achievement not motivation: robustness

current methods: 
Some existing works (cite KGCN, KGNNLS) use KG propagation, not explicit user-item propagation. 

Although others consider both, but they do not distinguish internal and external information with trustable and untrustable information. They equally treat all hetergeneous elements, which may lead to an unmatch or blurring epsecially for listwise recommendation task, e.g., TOP-K. (item - entity). 

1. summary problems: 1) user-item propagation (not fully exploit)  2) most existing work apply simple homogenous aggregation method. We hetergeous aggregation strategies (3) For item aggregation and entity aggregation, modeling not distinguish external knowledge 


our works: CF information fully trust-able, explicitly integrated external factual knowledge, we also propose case-level. summary, tackle problems: 1) user-item propogartion 2) attention more robust 3) CTR list-wise

In summary our contributions:
1) CF KG integration, distinguish Central role, integrate entrusted we proposed model..xxx
2) case-level attention, defense external noise, robustness
3) various acadmic, espically real world large-scale dataset MeiTuan, we extenslively claim



why user-item propagation is important.

2. KGAT and CKAN - KG propagation + explicit user-item propagation. They all

1. KGCN/KAT/CKAN
2. unify to CF/KG


1. internal aggregation (trustable information)
2. external aggregation + integrated aggregation (untrustable information)

Thus we do a case-level fine-grained attention mechanism for robust recommendation.  

20210119:
from HyperKGR:
significant test, such as Wilcoxon signed rank test (comparing our model performance under different seeds with the second best algorithm). Normally, we can say that: Bold values denote scenarios where a Wilcoxon signed rank test indicates a statistically significant difference between the best and second-best (underline) algorithms.


}
